Verifying Lock-free Search Structure Templates

We present and verify template algorithms for lock-free concurrent search structures that cover a broad range of existing implementations based on lists and skiplists. Our linearizability proofs are fully mechanized in the concurrent separation logic Iris. The proofs are modular and cover the broader design space of the underlying algorithms by parameterizing the verification over aspects such as the low-level representation of nodes and the style of data structure maintenance. As a further technical contribution, we present a mechanization of a recently proposed method for reasoning about future-dependent linearization points using hindsight arguments. The mechanization builds on Iris' support for prophecy reasoning and user-defined ghost resources. We demonstrate that the method can help to reduce the proof effort compared to direct prophecy-based proofs.

==> background.tex <==
\section{Motivation and Background}
\label{sec:background}

We motivate our work using a lockfree search structure called Michael Set from [cite]. The data structure implements a set ADT using a linked list. It provides three basic operations - search, insertion and deletion - of a key. This structure is particularly interesting because it corresponds to Herlihy's skiplist~\cite{AMP} when its height is restricted to just a single level. In this section, we discuss the algorithm, the intuitive proof idea and the challenges that arise when formalizing the proof idea.

\subsection{Algorithm for Michael set}


The algorithm, as presented here, abstracts away from node-level implementation details. [Add why].  The algorithm can be assumed to be executing on a set of node $N$. With each node $n$ is associated its key $\keyof{n} \in \keyspace = \mathbb{N} \cup \{\infty\}$, the next node it points to $\nextof{n} \in N$, and its mark bit $\markof{n} \in \{\true, \false\}$. The mark bit is used by the algorithm to \emph{logically} delete a node before physically removing it. These node level quantities can be read and updated via \emph{helper functions} such as \code{findNext}, \code{markNode}, etc. We additionaly assume two sentinel nodes head $\vhead$ and tail $\vtail$. The structure maintains invariant the following facts : $\keyof{\vhead} = 0$, $\keyof{\vtail} = \infty$, $\nextof{\vtail} = \vtail$, $\markof{\vhead} = \false$, $\markof{\vtail} = \false$.

\Cref{fig:lock-free-template} shows the Michael set algorithm. It encodes the mark bit by bit-stealing on the next pointer so as to verify that a node has not been logically deleted when changing its next pointer in a single atomic step. (A common technique when implementing lock-free structures). The algorithm can be instantiated by implementing the helper functions (highlighted in pink) that abstract from the node-level details. The helper functions are constrained to be \emph{logically atomic}, i.e., appear to take effect in a single step during its execution.

\begin{figure}
  \centering
  \begin{minipage}[t]{.50\textwidth}
\begin{lstlisting}[aboveskip=0pt,belowskip=0pt, frame=none]
let rec traverseRec $k$ $\vpred$ $\vcurr$ =
  match |<findNext>| $k$ $\vcurr$ with
  | $\vcurrnext$, true -> 
    match |<changeNext>| $\vpred$ $\vcurr$ $\vcurrnext$ with
    | Success -> traverseRec $k$ $\vpred$ $\vcurrnext$
    | Failure -> traverse $r$ $k$
  | $\vcurrnext$, false -> 
    match |<compareKey>| $\vcurr$ $k$ with
    | -1 => traverseRec $k$ $\vcurr$ $\vcurrnext$
    | 0 => ($\vpred$, $\vcurr$, true)
    | 1 => ($\vpred$, $\vcurr$, false)

let traverse $\vhead$ $\vtail$ $k$ =    
  match |<findNext>| $k$ $\vhead$ with 
  | $\vcurr$, _ -> traverseRec $k$ $\vhead$ $\vcurr$

let search $\vhead$ $\vtail$ $k$ =
  let _, _, $\vres$ = traverse $\vhead$ $\vtail$ $k$ in
  $\vres$
\end{lstlisting}
\end{minipage}%
\begin{minipage}[t]{.50\textwidth}
\begin{lstlisting}[aboveskip=0pt,belowskip=0pt, frame=none, firstnumber=last]
let insert $\vhead$ $\vtail$ $k$ =
  let $\vpred$, $\vcurr$, $\vres$ = traverse $\vhead$ $\vtail$ $k$ in
  if $\vres$ then
    false
  else
    let $\ventry$ = |<createNode>| $k$ $\vcurr$ in
    match |<changeNext>| $\vpred$ $\vcurr$ $\ventry$ with
    | Success -> true
    | Failure -> insert $\vhead$ $\vtail$ $k$ 
		
let delete $\vhead$ $\vtail$ $k$ =
  let $\vpred$, $\vcurr$, $\vres$ = traverse $\vhead$ $\vtail$ $k$ in
  if not $\vres$ then
    false
  else
    match |<markNode>| $\vcurr$ with @\label{line-delete-markNode}@
    | Success -> traverse $\vhead$ $\vtail$ $k$; true
    | Failure -> false
\end{lstlisting}
\end{minipage}
\caption{\label{fig:lock-free-template} Algorithm for the Michael set. The template can be instantiated by providing implementations of helper functions \code{findNext}, \code{changeNext}, \code{compareKey}, \code{createNode} and \code{markNode}. \code{findNext}$\,k\,\,\vcurr$ returns a pair $(\nextof{\vcurr}, \markof{\vcurr})$. \code{changeNext}$\,\vpred\,\,\vcurr\,\,\vcurrnext$ is a CAS operation attempting to change the next pointer of $\vpred$ from $\vcurr$ to $\vcurrnext$. \code{compareKey}$\,\vcurr\,\,k$ returns \code{-1} if $\keyof{\vcurr} < k$, \code{0} if $\keyof{\vcurr} = k$ and \code{1} otherwise. \code{maintainanceOp}$\,\vpred\,\vcurr\,\vcurrnext$ unlinks node $\vcurr$ out of the structure by redirecting edgeset from $\vpred$ to $\vcurrnext$. \code{createNode}$\,k\,\vcurr$ creates a new node $e$ containing $k$ whose edgeset is directed towards node $\vcurr$. Finally, \code{markNode}$\,\vcurr$ attempts to mark the $\vcurr$ node atomically, and failing if $\vcurr$ has been marked already. }
\end{figure}

Focusing on the algorithm now, \code{traverse} functions is the mainstay for all other operations \code{search}, \code{insert} and \code{delete}. The actual traversal is performed by recursive function \code{traverseRec}$\,k\,\,\vpred\,\,\vcurr$. It reads the mark bit and next pointer of $\vcurr$ using \code{findNext}. If $\vcurr$ is found to be marked, then \code{traverseRec} attempts to physically remove the node using \code{changeNext}. In case \code{changeNext} fails (because either $\vpred$ is marked or it does not point to $\vcurr$ anymore), it simply restarts from the $\vhead$ node. In case of \code{Success} of \code{changeNext}, the traversal continues. If $\vcurr$ is unmarked, then \code{traverseRec} proceeds by comparing $k$ to $\keyof{\vcurr}$. For $\keyof{\vcurr} < k$, the traversal continues with $\vcurr$ and $\vcurrnext$. Otherwise, the traversal ends at $\vcurr$, returning $(\vpred, \vcurr, true)$ if $\keyof{\vcurr} = k$ and $(\vpred, \vcurr, true)$ otherwise. To summarize, \code{traverse} performs physical deletion upon visiting a marked node, and it witnesses an unmarked $\vpred$ pointing to $\vcurr$ and that $\vcurr$ was unmarked at some point during its execution. 

The \code{search} operation simply invokes \code{traverse} function, whose result establishes where $k$ was in the structure or not. The \code{insert} operation starts by invoking \code{traverse} function. If the traversal returns true, then the key must already be present. Hence, \code{insert} returns $\false$ in this case. Otherwise, a new node $\ventry$ is created using \code{createNode} and an attempt is made to insert it into the list by \code{changeNext}. If the attempt succeeds, then \code{insert} returns with $\true$, else it restarts. Similar to \code{insert}, the \code{delete} operation also first checks if the key is present in the structure. If yes, then it attempts to mark $\vcurr$ via \code{markNode}. If marking succeeds, it returns \code{true} to indicate that deletion succeeded. Otherwise, a concurrent thread must have already deleted $k$, in which case \code{delete} returns \code{false}.

%A curios reader will notice that the algorithm believes that $k$ was not in the structure at some point during \code{traverse}'s execution in case it returns $\vres = false$. The crux of the linearizability proof of this structure indeed lies in establishing this fact. In the next section, we analyse the algorithm further and provide an intuitive proof of correctness.


\subsection{Proof Intuition}
\label{sec:proof-intuition}

\begin{figure}[h]
  \begin{align*}
  \dSpec{op}(k, C, C', \result)
  &\defeq
    \begin{cases}
      C' = C \land (\result \iff k \in C) & \cssOp = \code{search} \\
      C' = C \cup \set{k} \land (\result \iff k \not\in C) & \cssOp = \code{insert} \\
      C' = C \setminus \set{k} \land (\result \iff k \in C) & \cssOp = \code{delete}
    \end{cases}
  \end{align*}
  \caption{Sequential specification of a search structure. $k$ refers to the operation key, $C$ and $C'$ to the abstract state pre and post operation $\cssOp$ respectively and $\result$ is the final result.}
  \label{fig-search-str-spec}
\end{figure}

Our goal is to show that Michael's Set algorithm is linearizable. That is, we must prove that each of the operations (\code{search}, \code{insert}, and \code{delete}) takes effect in a single atomic step during its execution, the \emph{linearization point}, and satisfies the sequential specification shown in \Cref{fig-search-str-spec}. For our example, we define the abstract state $\contentsof{N}$ to be the union of \emph{logical contents} $\contentsof{n}$ of all nodes in $N$, where $\contentsof{n} \defeq \ite{\markof{n}}{\emptyset}{\{\keyof{n}\}}$. 

We aim for a proof strategy that is compatible with local reasoning principles and mostly agnostic to the detailed invariants of the specific data structure under consideration. The Edgeset and the Flow Framework from [cite] enter the picture here. The Edgset framework allows us to define \emph{keyset} of a node $\keysetof{n}$, intuitively capturing the set of all keys that $n$ is responsible for. Consider \Cref{fig:keyset-intuition} for instance, a thread executing \code{search(6)} without any interference will reach node $n_4$ and terminate, concluding that $6$ is not present in the structure. In this sense, we say $n_4$ is responsible for key $6$ and is part of its keyset. The keysets partition the set of all keys and provide the following crucial property : for any node $n$ and key $k$, 
\[k \in \keysetof{\anode} \Rightarrow (k \in \contentsof{N} \Leftrightarrow k \in \contentsof{\anode})\enspace.\]
This property allows us to reduce the correctness of an insertion, deletion, and search for $k$ on the global abstract state $\contentsof{N}$ to the correctness of the same operation on $\anode$'s local contents $\contentsof{\anode}$, provided we can show $k \in \keysetof{\anode}$. For example, suppose that a concurrent invocation of \code{delete($k$)} returns \code{false}. To prove that this invocation is linearizable, one has to show that at some point during \code{delete($k$)}'s execution, $k$ was not contained in the structure. With keysets, it suffices to show that there exists a node $\anode$ such that both $k \in \keysetof{\anode}$ and $k \notin \contentsof{\anode}$ were true at the same point in time during \code{delete($k$)}'s execution. We refer to $\anode$ as the decisive node of the operation. The point in time where the two facts about $\anode$ hold is the linearization point.

The keyset is an inductive quantity defined on the global data structure graph. The flow framework allows one to reason about such inductive quantities in a local manner using techniques based on Separation Logic. We defer details about how to encode keysets to the later part of this section.

\begin{figure}[t]
\centering
  \begin{tikzpicture}[>=stealth, font=\footnotesize, scale=1, every node/.style={scale=0.8}]
    % Nodes
  \def\xsep{1.5}
  \def\ysep{-1.8}

    \node[unode] (hd) {$0$};
    \node[stackVar, below=0.1mm of hd] (hd') {$\vhead$};

    \node[unode, right=6mm of hd] (n2) {$2$};
    \node[stackVar, below=0.1mm of n2] (n2') {$n_1$};

    \node[mnode, right=6mm of n2] (n4) {$4$};
    \node[stackVar, below=0.1mm of n4] (n4') {$n_2$};
    \node[mnode, right=6mm of n4] (n7) {$7$};
    \node[stackVar, below=0.1mm of n7] (n7') {$n_3$};
    \node[unode, right=6mm of n7] (n9) {$9$};
    \node[stackVar, below=0.1mm of n9] (n9') {$n_4$};
    \node[mnode, right=6mm of n9] (n15) {$15$};
    \node[stackVar, below=0.1mm of n15] (n15') {$n_5$};

    \node[unode, right=6mm of n15] (tl) {$\infty$};
    \node[stackVar, below=0.1mm of tl] (tl') {$\vtail$};

    \node[mnode, above=5mm of n9] (n9new) {$9$};

    %\node[stackVar, below=.4cm of n4] (pred) {$\vpred$};
    %\node[stackVar, below=.4cm of n7] (curr) {$\vcurr$};

    % Edges
    %\draw[edge] (pred) to (n4);
    \draw[edge] (hd) to (n2);
    \draw[edge] (n2) to (n4);
    \draw[edge] (n4) to (n7);
    \draw[edge] (n7) to (n9);
    \draw[edge] (n9) to (n15);
    \draw[edge] (n15) to (tl);
    \draw[edge] (n9new) to (n15);
    %\draw[edge] (curr) to (n7);
    
    %\draw ($(inf.north west)+(-.3,1.4)$) rectangle ($(Inf.south east)+(.3,-1)$);

\end{tikzpicture}
  \caption{Possible state of the Michael's Set. The keyset of a marked node is always $\emptyset$. $\keysetof{\vhead} = \{0\}$, $\keysetof{n_1} = (0, 2]$, $\keysetof{n_9} = (2, 9]$ and $\keysetof{\vtail} = (9, \infty)$. In context of linked-lists, the keyset of a node is set of all keys greater than the key of its first unmarked predecessor and less than or equal to its own key.
  \label{fig:keyset-intuition}}
\end{figure}

Let us now turn to the proof of linearizability. The strategy is to identify the linearization point and decisive node $\anode$ for an operation on key $k$ by establishing the relevant facts about $k$'s membership in the keyset and contents of $\anode$. The key challenge here is that the linearization point of an operation may depend on concurrent operations performed by other threads. 

We discuss this issue using the \code{delete} operation. Consider threads $T_1$ and $T_2$ both executing \code{delete($7$)}, and thread $T_i$ executing \code{insert($7$)} concurrently. \Cref{fig:michael-set-state} shows two possible states observed during an interleaved execution of these threads. Initially, the structure contains values $4$, $7$ and $9$. The right-hand side depicts the state of $T_1$ at the point when its traversal has terminated after reaching node $n_2$.  Thread $T_1$ is now interrupted by $T_2$ which does its traversal and overtakes $T_1$ by successfully marking $n_2$. Then the traversal by $T_i$ unlinks $n_2$ from the structure and reinserts $7$ in a new node $n_4$. At this point $T_1$ resumes by executing \code{markNode} which fails because $n2$ is marked now. $T_1$ terminates by returning $\code{false}$ to indicate that $7$ is not in the structure. Although $7$ is present in the structure at the point when $T_1$ returns, this execution is  linearizable, because there existed a point in time when $7$ was not in the structure, namely right after $T_2$ marked node $n_2$.  %That is the linearization point of $T_1$. We further say that this is a \emph{pure} linearization point, as the abstract state of the structure does not change at this point.

\begin{figure}[t]
\centering
  \begin{tikzpicture}[>=stealth, font=\footnotesize, scale=1, every node/.style={scale=0.8}]
    % Nodes
  \def\xsep{1.5}
  \def\ysep{-1.8}

  \begin{scope}[local bounding box=g1]
    \node[unode] (inf) {$-\infty$};
    \node[stackVar, above=0.1mm of inf] (inf') {$r$};

    \node[unode, right=6mm of inf] (n4) {$4$};
    \node[stackVar, above=0.1mm of n4] (n4') {$n_1$};
    \node[unode, right=6mm of n4] (n7) {$7$};
    \node[stackVar, above=0.1mm of n7] (n7') {$n_2$};
    \node[unode, right=6mm of n7] (n9) {$9$};
    \node[stackVar, above=0.1mm of n9] (n9') {$n_3$};

    \node[unode, right=6mm of n9] (Inf) {$\infty$};
    \node[stackVar, above=0.1mm of Inf] (Inf') {$t$};

    \node[unode, white, above=5mm of n7] (n7new) {$7$};

    \node[stackVar, below=.4cm of n4] (pred) {$\vpred$};
    \node[stackVar, below=.4cm of n7] (curr) {$\vcurr$};

    % Edges
    \draw[edge] (pred) to (n4);
    \draw[edge] (inf) to (n4);
    \draw[edge] (n4) to (n7);
    \draw[edge] (n7) to (n9);
    \draw[edge] (n9) to (Inf);
    
    \draw[edge] (curr) to (n7);
    
    \draw ($(inf.north west)+(-.3,1.4)$) rectangle ($(Inf.south east)+(.3,-1)$);
  \end{scope}

  \begin{scope}[local bounding box=g2, shift={($(g1.east)+(2.8,-0.2)$)}]
    \node[unode] (inf) {$-\infty$};
    \node[stackVar, above=0.1mm of inf] (inf') {$r$};
    %\node[unode, right=5mm of inf] (n1) {$1$};
    %\node[mnode] (n2) at ($(n1) + (0, -\ysep/1.5)$) {$2$};
    \node[unode, right=6mm of inf] (n4) {$4$};
    \node[stackVar, above=0.1mm of n4] (n4') {$n_1$};
    %\node[mnode, right=6mm of n4] (n6) {$6$};
    \node[mnode, right=6mm of n4] (n7) {$7$};
    \node[stackVar, above=0.1mm of n7] (n7') {$n_2$};
    \node[unode, right=6mm of n7] (n9) {$9$};
    \node[stackVar, above=0.1mm of n9] (n9') {$n_3$};
    \node[unode, above=5mm of n7] (n7new) {$7$};
    \node[stackVar, right=1mm of n7new] (n7new') {$n_4$};
    \node[unode, right=6mm of n9] (Inf) {$\infty$};
    \node[stackVar, above=0.1mm of Inf] (Inf') {$t$};

    \node[stackVar, below=.4cm of n4] (pred) {$\vpred$};
    \node[stackVar, below=.4cm of n7] (curr) {$\vcurr$};

    % Edges
    \draw[edge] (pred) to (n4);
    \draw[edge] (inf) to (n4);
    %\draw[edge] (n4) to (n7);
    \draw[edge] (n7) to (n9);
    \draw[edge] (n9) to (Inf);
    
    \draw[edge] (n4) to[bend left=20] (n7new);
    \draw[edge] (n7new) to[bend left=20] (n9);
    %\draw[edge] (p) to (n3);
    \draw[edge] (curr) to (n7);
    \draw ($(inf.north west)+(-.3,1.4)$) rectangle ($(Inf.south east)+(.3,-1)$);

  \end{scope}

  \draw[edge,dotted] ($(g1.east)+(0,0)$) to node[above] {\large\begin{tabular}{l}\code{delete}$\,r\,7$\\\;\rotatebox[origin=c]{270}{$\rightsquigarrow$}\end{tabular}} node[below] {\large\begin{tabular}{r}\rotatebox[origin=c]{90}{$\rightsquigarrow$}\;\\\code{insert}$\,r\,7$\end{tabular}} ($(g2.west)+(0,0)$);

\end{tikzpicture}
  \caption{Two possible states of \code{delete($7$)} instantiated for linked lists. 
  Nodes are labeled with the value of their \code{key} field. Edges indicate \code{next} pointers. Marked (logically deleted) nodes are shaded gray. The left graph shows the state at the first invocation of \code{traverseRec}. The right graph shows the state at the last invocation of \code{traverseRec}. The traversal is interleaved with concurrent invocations of \code{delete($7$)} and \code{insert($7$)}.
  \label{fig:michael-set-state}}
\end{figure}

Contrast the above case with an execution of $T_1$ that is not interleaved by any other threads. In this case, the $T_1$ would successfully mark node $n_2$ and return $\code{true}$. 

The linearizability argument of the \code{delete} can be summarized as follows. First, we can establish using an inductive argument that node $n$ returned by \code{traverse} was unmarked and had $k$ in its keyset at some point during \code{traverse}'s execution, and that $\vres$ is true iff $k = \keyof{\vcurr}$. If $\vres$ is \code{false}, then the time point when \code{traverse} observed the two facts about $n$ becomes its linearization point. Otherwise, \code{delete} attempts to mark $n$ using \code{markNode}. Either it succeeds and this atomic step becomes its linearization point; or it fails, meaning a concurrent interfering thread marked $n$ between the end of \code{traverse} and the attempted marking. In the failing case, the linearization point is when the other thread marks $n$, and this point is already past. The thread executing \code{delete} may not directly observe this point, but it can however establish its existence in hindsight.

%Formalizing above proof argument in Iris is challenging. 
In order to prove linearizability in Iris, one has to pinpoint the exact point of linearization for all cases of all operations. However, as in the case of future-dependent linearzation point of \code{delete}, the linearization point is only clear in hindsight once it has passed. To deal with such a scenario, one needs to use prophecy variables.

The thread executing \code{delete} for instance could prophesize whether \code{markNode} will succeed or fail, and use that information to perform case-analysis similar to the intuitive proof above. This is further complicated by the fact that a linearization point could lie outside of the operation under consideration (as is the case with \code{delete}). To deal with this, one needs to devise a \emph{helping protocol} that facilitates transfer of linearizability obligation between concurrent threads. Devising such a protocol entails specifying details such as which thread must linearize which, when does a thread need \emph{helping} vs.\ when it does not, etc. 

Such details differ greatly when one considers disparate structures like LSM trees and lockfree linked-lists like Michael's Set above. Hence, even though the underlying linearizability arguments via hindsight are simple for such structures, devising the helping protocol is more than half the work and needs rework for each structure separately. 

Hindsight reasoning enables temporal reasoning about computations using \emph{past predicates}, which express that a \emph{state predicate} held true at some prior state of the computation. We refer to the general proof principle behind hindsight theory as \emph{temporal interpolation}. That is, one proves lemmas of the form: if there existed a past state that satisfied property $p$ and the current state satisfies $q$, then there must have existed an intermediate state that satisfied $o$. Such lemmas can then be applied, e.g., to prove that if \code{delete}'s traversal observed $n$ to be unmarked and later $n$ is found to be marked before \code{markNode}, then it must have been marked at some point in between\footnote{The structure holds invariant that a node once marked remains marked.}. It is clear how such a lemma implies the existence of a linearization point of \code{delete} in hindsight.

In the next section, we devise an encoding that provides support for hindsight reasoning in Iris by devising a generic helping protocol that work for a broad class of structures we consider in this paper. The encoding will rely on the availability of prophecies and user-definable ghost resources. Finally, we use the encoding to relate the linearizability in hindsight with the notion of exact linearizability. This encoding of hindsight is a one-time construction that is not exposed to the user of the encoding. The user has to establish only the existence of linearization point in order to prove exact linearizability for an operation.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "description"
%%% End:


==> status.tex <==
\section{Status of Proposed Work}

%\twcomment{You may want to summarize the parts from the earlier papers that will become part of the thesis. You can change the title of the section to "Status of Proposed Work" or similar.}

Along with the ideas presented in this proposal, our earlier work on verifying lock-based search structure templates~\cite{DBLP:journals/pacmpl/PatelKSW21, DBLP:conf/pldi/KrishnaPSW20} will also become part of the proposed thesis. We begin by summarizing my contribution to those projects here. The work in~\cite{DBLP:conf/pldi/KrishnaPSW20} focuses on verifying lock-based single-copy structures, i.e., search structures which have atmost one copy of a key in the structure\footnote{Put differently, search structures with \emph{in-place} update design.}. Search structures considered in~\cite{DBLP:conf/pldi/KrishnaPSW20} include (lock-based) variants of B-trees, hash tables and linked lists. The main theoretical contribution in~\cite{DBLP:conf/pldi/KrishnaPSW20} that will be part of this proposed thesis is the novel \emph{keyset} resource algebra that allows reasoning at the node-level to be lifted at the search structure level. This resource algebra facilitates the mechanization in Iris of ideas presented in~\refSec{sec:proof-intuition}.

In~\cite{DBLP:journals/pacmpl/PatelKSW21}, we expand the methodology developed in~\cite{DBLP:conf/pldi/KrishnaPSW20} to multicopy structures, i.e. search structures containing possibly multiple copies of the same key\footnote{These structures follow the \emph{out-of-place} update design.}. Search structures considered here are implementations of the Log-Structured Merge Trees. The main theoretical contribution of this work is reframing the client-level specification into a \emph{Search Recency} specification that admits simpler linearizability proofs. The proof relating the client-level specification to Search Recency can be reused across all templates. The ideas in~\refSec{sec-hindsight} can be viewed as a generalization of the methodology presented in~\cite{DBLP:journals/pacmpl/PatelKSW21}. This work will be included in full and form a chapter of the proposed thesis.    

We break down the remaining work towards verifying lock-free templates into following high-level steps.
\begin{enumerate}
    \item Implement the proof relating hindsight specifications with the client-level specifications.
    \item Prove the hindsight specifications for \emph{simpler} search structure templates, like the Michael's set presented in this proposal. Other variations depending on whether the traversal is wait-free or not are possible. The proof for such templates is similar to the one presented in this paper.
    \item Prove the hindsight specifications for templates covering concurrent skiplists. Several variants are possible here, depending on whether the traversal is wait-free or not and the direction of marking. 
    \item Explore a generic lock-free template that covers both, skiplists and simpler linked list implementations like Michael's set and Harris List.  
    \item Extend the presented methodology to multicopy lock-free templates, like the BW-tree~\cite{DBLP:conf/icde/LevandoskiLS13a} for instance.
\end{enumerate}
%\twcomment{Isn't there also still work to be done on coming up with the generic lock-free templates?}

We have accomplished step (1), and currently we are working on proving the hindsight specification for the simplified skiplist (step (2)). The next step will be to extend the template presented here to a template describing skiplists. Proving hindsight specifications for skiplist template will result in a formally verified concurrent skiplist. Presently, we have an early version of a template for Herlihy's skiplist~\cite{AMP} and a paper proof of its hindsight specification. We also intend to verify a simplified version of lock-free concurrent skiplist implementation from \texttt{java.util.concurrent.ConcurrentSkipListSet}~\cite{java-skiplist}.

We include steps (4) and (5) as stretch goals. In (4), we conjecture a lock-free template that covers skiplists and simpler linked list implementations. This is based on the intuition that only operations on the \emph{base} list of the skiplist change the abstract state of the structure. The operations on higher levels in the skiplist can thus be considered as \emph{maintainence}, which is simply absent in simpler linked list implementations. This paves a way forward to view these two classes of search structures in a uniform manner.  

We believe that the work presented in this proposal can be extended to multicopy lock-free structures as well. This is the subject of exploration in step (5). We also believe that the proofs in the final form of our current project should significantly simplify proofs from our earlier work on lock-based multicopy structures~\cite{DBLP:journals/pacmpl/PatelKSW21}. 

